Bayesian Neural Scaling Law Extrapolation with Prior-Data Fitted Networks

Scaling has been a major driver of recent advancements in deep learning. Numerous empirical studies have found that scaling laws often follow the power-law and proposed several variants of power-law functions to predict the scaling behavior at larger scales. However, existing methods mostly rely on point estimation and do not quantify uncertainty, which is crucial for real-world applications involving decision-making problems such as determining the expected performance improvements achievable by investing additional computational resources. In this work, we explore a Bayesian framework based on Prior-data Fitted Networks (PFNs) for neural scaling law extrapolation. Specifically, we design a prior distribution that enables the sampling of infinitely many synthetic functions resembling real-world neural scaling laws, allowing our PFN to meta-learn the extrapolation. We validate the effectiveness of our approach on real-world neural scaling laws, comparing it against both the existing point estimation methods and Bayesian approaches. Our method demonstrates superior performance, particularly in data-limited scenarios such as Bayesian active learning, underscoring its potential for reliable, uncertainty-aware extrapolation in practical applications.

==> captions/fig_cutoff_RMSLE.tex <==
\begin{figure*}[h]
\vspace{-0.1in}
\includegraphics[height=0.6cm]{figures/legend1.pdf}
\medskip
\vspace{-0.14in}
\centering
\includegraphics[width=0.245\textwidth]{figures/IC_RMSLE.pdf}
\includegraphics[width=0.245\textwidth]{figures/NLP_RMSLE.pdf}
\includegraphics[width=0.245\textwidth]{figures/ColPret_RMSLE.pdf}
\includegraphics[width=0.245\textwidth]{figures/DD_RMSLE.pdf}
\vspace{-0.2in}
\caption{\small \textbf{Extrapolation performance (RMSLE) with varying cutoffs}. 
%We clip extremely low log-likelihood values to enhance presentation clarity of the figure. 
%Note that we exclude the result of MCMC (BNSL) in the 20\% setting, as the context size is too small to validate the number of breaks.
}
\label{fig:cutoff_RMSLE}
\end{figure*}
